Fast and Accurate Proper Orthogonal Decomposition using Efficient Sampling and Iterative Techniques for Singular Value Decomposition

In this paper, we propose a computationally efficient iterative algorithm for proper orthogonal decomposition (POD) using random sampling based techniques. In this algorithm, additional rows and columns are sampled and a merging technique is used to update the dominant POD modes in each iteration. We derive bounds for the spectral norm of the error introduced by a series of merging operations. We use an existing theorem to get an approximate measure of the quality of subspaces obtained on convergence of the iteration. Results on various datasets indicate that the POD modes and/or the subspaces are approximated with excellent accuracy with a significant runtime improvement over computing the truncated SVD. We also propose a method to compute the POD modes of large matrices that do not fit in the RAM using this iterative sampling and merging algorithms.

==> 7speedup.tex <==
\begin{figure}[tbhp!]
  \begin{minipage}{\textwidth}
    \centering
    \ref{spd_US}
  \end{minipage}\\
  \begin{minipage}{\textwidth}
    \centering
    Single thread\\
     \scalebox{0.75}{
       \input{figures/tikz_barplot_speedup_US_V_2D_single_thread.tex}}
     \scalebox{0.75}{
       \input{figures/tikz_barplot_speedup_US_faces_single_thread.tex}}
      \scalebox{0.75}{
        \input{figures/tikz_barplot_speedup_US_croppedYalefaces_single_thread.tex}}\\
     \end{minipage}
  \begin{minipage}{\textwidth}
    \centering
    4 threads\\
     \scalebox{0.75}{
       \input{figures/tikz_barplot_speedup_US_V_2D_4_threads.tex}}
      \scalebox{0.75}{
       \input{figures/tikz_barplot_speedup_US_faces_4_threads.tex}}
      \scalebox{0.75}{
       \input{figures/tikz_barplot_speedup_US_croppedYalefaces_4_threads.tex}}
  \end{minipage}
  \caption{Speed up obtained due to using unique sampling algorithms with respect to LTSVD, CTSVD and SVD($A^TA$) when run on different datasets for different parameter values, as given in Table~\ref{tab:parval}.} %Plots on the left show speed up computed from CPU time. Plots on the right show speed up computed from elapsed time.}
  \label{fig:speedup_US}
\end{figure}




==> LTSVD_US.tex <==

%---------------------------------------LTSVD-US-------------------------------
%---------------------------------------LTSVD-US-------------------------------
\begin{algorithm}[!htbp]
  \small
  \caption{ 
  Inputs: matrix $A \in \mathbb{R}^{m\times n}$,  
  number of columns/rows to be sampled $c/w$  and
   rank of approximation, $k$, 
  sampling probabilities for columns and rows, $\bv{p},\bv{q}$}
  \label{alg:LTSVD_US}
  \begin{algorithmic}[1]
    \Procedure{Sample and Scale Unique Columns}{$A$, $\bv{p}$, $c$}
    \State $\bv{I}_s \gets s_i \text{ containing $c$ column indices sampled with probability } \bv{p}$
    \State $\bv{I}_c\gets s_i ; \bv{t}\gets \{t_i, \text{ number of occurrences of }s_i \} :\forall \text{ distinct } s_i\in \bv{I}_s $
    \State $g\gets card(\bv{I}_c)$ \Comment {Cardinality of the set}
    \State $\bv{c}_i \gets \bv{a}_{\eta_i}\sqrt{t_i/(cp_{\eta_i})},\text{ where }\eta_i\in\bv{I}_c \text{ and }
    i=1,2,\cdots,g$  
      \State \textbf{return} $C$
      \EndProcedure
  \Procedure {Sample and Scale Unique Rows}{$C,\bv{q},w$}
  \State $\bv{\hat{I}}_s\gets \hat{s}_j \text{ containing $w$ row indices sampled with probability  }
  \bv{q}$
  \State $\bv{I}_r\gets \hat{s}_j; \bv{\hat{t}}\gets \{\hat{t}_i, \text{ number of occurrences of }\hat{s}_j \}:\forall \text{ distinct } \hat{s}_j\in \bv{\hat{I}}_s $
  \State $h\gets card(\bv{I}_r)$
  \State $\bv{w}^i \gets \bv{c}^{\xi_i}\sqrt{\hat{t}_i/(wq_{\xi_i})},\text{ where }\xi_i\in\bv{I}_r \text{ and }i=1,2,\cdots,h$    
  \State \textbf{return} {$W$}
  \EndProcedure
  \end{algorithmic}
  
\end{algorithm}

